Deep Learning on Graphs for Mobile Network Topology Generation

Mobile networks consist of interconnected radio nodes strategically positioned across various geographical regions to provide connectivity services. The set of relations between these radio nodes, referred to as the \emph{mobile network topology}, is vital in the construction of the networking infrastructure. Typically, the connections between radio nodes and their associated cells are defined by software features that establish mobility relations (referred to as \emph{edges} in this paper) within the mobile network graph through heuristic methods. Although these approaches are efficient, they encounter significant limitations, particularly since edges can only be established prior to the installation of physical hardware. In this work, we use graph-based deep learning methods to determine mobility relations (edges), trained on radio node configuration data and reliable mobility relations set by Automatic Neighbor Relations (ANR) in stable networks. This paper focuses on measuring the accuracy and precision of different graph-based deep learning approaches applied to real-world mobile networks. We evaluated two deep learning models. Our comprehensive experiments on Telecom datasets obtained from operational Telecom Networks demonstrate the effectiveness of the graph neural network (GNN) model and multilayer perceptron. Our evaluation showed that considering graph structure improves results, which motivates the use of GNNs. Additionally, we investigated the use of heuristics to reduce the training time based on the distance between radio nodes to eliminate irrelevant cases. Our investigation showed that the use of these heuristics improved precision and accuracy considerably.

==> sections/00_abstract.tex <==
\begin{abstract}
Mobile cellular networks are widely integrated in today's infrastructure. These networks are constantly evolving and continuously expanding, especially with the introduction of fifth-generation (5G). It is important to ensure the effectiveness of these expansions. 

Mobile networks consist of a set of radio nodes that are distributed in a geographical region to provide connectivity services. Each radio node is served by a set of cells. The handover relations between cells is determined by Software features such as Automatic Neighbor Relations (ANR). The handover relations, also refereed as edges, between radio nodes in the mobile network graph are created through historical interactions between User Equipment (UE) and radio nodes. The method has the limitation of not being able to set the edges before the physical hardware is integrated. In this work, we use graph-based deep learning methods to determine mobility relations (edges), trained on radio node configuration data and a set of reliable relations of ANR in stable networks. The report focuses on measuring the accuracy and precision of different graph based deep learning approaches applied to real-world mobile networks. The report considers four models. Our comprehensive experiments on Telecom datasets obtained from operational Telecom Networks demonstrate that graph neural network model and multilayer perceptron trained with Binary Cross Entropy (BCE) loss outperform all other models.  The four models evaluation showed that considering graph structure improve results. Additionally, the model investigates the use of heuristics to reduce the training time based on distance between radio node to eliminate irrelevant cases. The use of these heuristics improved precision and accuracy.
\end{abstract}

\begin{IEEEkeywords}
TelcoAI, AI for 5G-and-beyond networks
\end{IEEEkeywords}

==> sections/01_intro.tex <==
\section{Introduction}
Mobile networks are the backbone of communications today and are widely integrated in large parts of society. These networks consist of connections between different radio nodes (base stations). Each radio node provides connectivity coverage to end-user equipment (UE). UEs is a device with connectivity capabilities such as smart phones, watches or smart cars. One of the key functions in a mobile network is the concept of a handover. A handover is the transfer of connection from radio node to another. In 5G/NR and 4G/LTE networks, handovers are made possible by maintaining a fixed cell relation list \cite{Cloud_based_link_prediction} which provide possible neighboring radio nodes that a UE connects to when moving from a coverage area to another. 

This thesis details evaluates multiple deep learning models to generate cell relations before deployment of new cells and base stations using attribute information from the network. This has been tried and studied previously in \cite{Cloud_based_link_prediction},\cite{dahlen11},\cite{automatic_cell_list_def07} %add more sources
among others. A successful approach that is implemented today is a technology named ANR (automated neighbour relations) \cite{dahlen11}. ANR uses network traffic through the movement of UEs in the network and handover statistics among other data to find the neighbours. Consequently, ANR can only be used after deployment of radio node or cells and that the process of deciding the initial cell relations might be slow. The aim of this thesis is to find these relations for new radio nodes using information that is available before deployment. The closest work we found was \cite{Cloud_based_link_prediction}. To address this challenge, we represent a mobile network as a graph and formulate the problem as an inductive link prediction task. Previous work on inductive link prediction showed success in using artificial neural networks, and more specifically graph neural networks as seen in \cite{DEAL},\cite{G2G},\cite{graph2Feat}. Inspired by these efforts and the wide applications of machine learning in the telecommunications domain\cite{ML_telecom17} graph neural networks will be utilized in this work.

==> sections/02_related_work.tex <==
\section{Background}

==> sections/03_method.tex <==
\section{Method}

==> sections/04_experiments.tex <==
\section{Experiments}

==> sections/05_conclusion.tex <==
\section{Conclusion}
